QMDB: Quick Merkle Database

Quick Merkle Database (QMDB) addresses longstanding bottlenecks in blockchain state management by integrating key-value (KV) and Merkle tree storage into a single unified architecture. QMDB delivers a significant throughput improvement over existing architectures, achieving up to 6X over the widely used RocksDB and 8X over NOMT, a leading verifiable database. Its novel append-only twig-based design enables one SSD read per state access, O(1) IOs for updates, and in-memory Merkleization on a memory footprint as small as 2.3 bytes per entry, enabling it to run on even modest consumer-grade PCs. QMDB scales seamlessly across both commodity and enterprise hardware, achieving up to 2.28 million state updates per second. This performance enables support for 1 million token transfers per second (TPS), marking QMDB as the first solution achieving such a milestone. QMDB has been benchmarked with workloads exceeding 15 billion entries (10X Ethereum's 2024 state) and has proven the capacity to scale to 280 billion entries on a single server. Furthermore, QMDB introduces historical proofs, unlocking the ability to query its blockchain's historical state at the latest block. QMDB not only meets the demands of current blockchains but also provides a robust foundation for building scalable, efficient, and verifiable decentralized applications across diverse use cases.

==> unused_sections/related.tex <==
\section{Related work}
\label{sec:related}
% \paragraph{Merkle key-value stores in blockchains.} We categorize blockchain execution clients by the architecture of their storage layers. Two-layer architectures are most common, where a merklization layer is built on top of a general-purpose key-value store. We further divide clients by the internal data structure they used for their ADS. Merkle Patricia tries are used in Geth [cite], while others (Merk [cite], IAVL [cite]) have adopted AVL trees and their variants for more efficient proof creation and verification on key ranges. One-layer architectures (such as that used in QMDB) improve upon two-layer architectures by storing the authenticated data structure natively on storage media. Existing implementations such as NOMT [cite], Firewood [cite] and MonadDB [cite] have tried to optimize for larger state sizes. However, all existing solutions have no choice but to resort to SSD storage to cope with realistic larger state sizes. QMDB is the first solution that can perform merklization using only in-memory data while using SSD as its backing store, meaning it is much faster for real-life state sizes.


% \paragraph{Adapting general-purpose key-value stores for blockchains.} Earlier work focused on optimizing the databases relied on in two-layer architectures. These databases may internally use LSM trees (LevelDB~\cite{}, RocksDB~\cite{}) or B-trees (MDBX~\cite{}). Storing an authenticated data structure in these databases causes significant read and write amplification. Optimizations include the batching of writes (ParityDB~\cite{}, MoltDB~\cite{}).
% MoltDB segregated states by recency and introduced a compaction process to reduce disk I/O and increase throughput by 30%~\cite{liang2024moltdb}.


% \paragraph{Orthogonal optimizations for merkle tree computation.} Several techniques have been explored for accelerating the expensive step of merkle tree computation, such as caching~\cite{el2023towards,dahlberg2016efficient}, optimizing subtrees~\cite{ayyalasomayajula2023optimization}, and using specialized hardware~\cite{jeon2023hardware,deng2024accelerating}. zkTrie~\cite{} uses zk-friendly hash functions to be zk-friendly itself by composition. These are orthogonal improvements and could be applied in conjunction with QMDB.

% \paragraph{Verifiable ledger databases.}
% These are systems that allow users to verify that a log is indeed append-only, of which blockchains are a subset. Deferred verification is a common approach~\cite{glass,ledger,sqlledger}. GlassDB~\cite{yue2022glassdb} uses a POS-tree (a Merkle tree variant) as an ADS for efficient proofs. Amazon’s QLDB~\cite{}, Azure’s SQLLedger~\cite{}, and Alibaba’s LedgerDB~\cite{} are commercially available verifiable databases that use Merkle trees (or variants) internally to provide transparency logs. VeritasDB uses trusted hardware (SGX) to aid verification~\cite{}. The key difference between such databases and systems like QMDB is that the latter are optimized for frequent state updates and real-time verification of the current state (as opposed to verification of historical logs and deferred verification).

**Merkle key-value stores in blockchains.** We categorize blockchain execution clients by the architecture of their storage layers. *Two-layer architectures* are most common, where a merklization layer is built on top of a general-purpose key-value store. We further divide clients by the internal data structure they used for their ADS. Merkle Patricia tries are used in Geth \[cite\], while others (Merk \[cite\], IAVL \[cite\]) have adopted AVL trees and their variants for more efficient proof creation and verification on key ranges. *One-layer architectures* (such as that used in QMDB) improve upon two-layer architectures by storing the authenticated data structure natively on storage media. Existing implementations such as NOMT \[cite\], Firewood \[cite\] and MonadDB \[cite\] have tried to optimize for larger state sizes. However, all existing solutions have no choice but to resort to SSD storage to cope with realistic larger state sizes. QMDB is the first solution that can perform merklization using only in-memory data while using SSD as its backing store, meaning it can handle the state sizes of even larger blockchains such as Ethereum.

| System | \#Layers | Merkle nodes stored in | Internal data structure | Open-source | Description |
| :---- | :---- | :---- | :---- | :---- | :---- |
| QMDB | 1 | DRAM | B-tree | Yes | This paper. |
| [NOMT](https://github.com/thrumdev/nomt) | 1 | SSD | Trie | [Yes](https://github.com/thrumdev/nomt) | 40k TPS on 128M accounts. Targeting 25k TPS with 1 billion by EOY 2024\. |
| [Firewood](https://www.avax.network/blog/introducing-firewood-a-next-generation-database-built-for-high-throughput-blockchains) | 1 | SSD | Trie | [Yes](https://github.com/ava-labs/firewood) |  |
| NomadDB | 1 | SSD | ?? | No |  |
| [MonadDB](https://docs.monad.xyz/technical-discussion/execution/monaddb) | 1 | SSD | Patricia trie | No? | 10,000 “real TPS” claimed |
| [Merk](https://github.com/turbofish-org/merk) | 2 | Database (RocksDB) | AVL | [Yes](https://github.com/turbofish-org/merk) | Merkle AVL \+ RocksDB |
| [IAVL+](https://github.com/cosmos/iavl) (Cosmos) | 2 | Database (GoLevelDB) | AVL | [Yes](https://github.com/cosmos/iavl) |  |
| [Geth](https://github.com/ethereum/go-ethereum) \[[Wood14](https://ethereum.github.io/yellowpaper/paper.pdf)\] | 2 | Database (LevelDB) | Patricia trie | [Yes](https://www.google.com/url?q=https://github.com/ethereum/go-ethereum&sa=D&source=docs&ust=1732300916146898&usg=AOvVaw1qAOqsategKly1Nt_Cp2xP) | Official Ethereum execution client |
| [JMT](https://developers.diem.com/docs/technical-papers/jellyfish-merkle-tree-paper/) \[[Gao21](https://developers.diem.com/papers/jellyfish-merkle-tree/2021-01-14.pdf)\] | 2 | Database (RocksDB) | Patricia trie variant | [Yes](https://github.com/diem/diem/tree/main/storage/jellyfish-merkle) |  |
| MoltDB  \[[Liang24](https://ieeexplore.ieee.org/abstract/document/10713891)\] | 2 | Database (LevelDB) | Patricia trie | No |  |

**Adapting general-purpose key-value stores for blockchains.** Earlier work focused on optimizing the databases relied on in two-layer architectures. These databases may internally use LSM trees (LevelDB\~\\cite{}, RocksDB\~\\cite{}) or B-trees (MDBX\~\\cite{}). Storing an authenticated data structure in these databases causes significant read and write amplification. Optimizations include the batching of writes (ParityDB\~\\cite{}, MoltDB\~\\cite{}).  
MoltDB segregated states by recency and introduced a compaction process to reduce disk I/O and increase throughput by 30%\~\\cite{liang2024moltdb}.

**Orthogonal optimizations for merkle tree computation.** Several techniques have been explored for accelerating the expensive step of merkle tree computation, such as caching\~\\cite{el2023towards,dahlberg2016efficient}, optimizing subtrees\~\\cite{ayyalasomayajula2023optimization}, and using specialized hardware\~\\cite{jeon2023hardware,deng2024accelerating}. zkTrie\~\\cite{} uses zk-friendly hash functions to be zk-friendly itself by composition. These are orthogonal improvements and could be applied in conjunction with QMDB.

\[Mention Verkle trees as an attempt to overcome MPT?\]  

Verifiable ledger databases. These are systems that allow users to verify that a log is indeed append-only, of which blockchains are a subset. Deferred verification is a common approach~\cite{glass,ledger,sqlledger}. GlassDB~\cite{yue2022glassdb} uses a POS-tree (a Merkle tree variant) as an ADS for efficient proofs. Amazon’s QLDB~\cite{}, Azure’s SQLLedger, and Alibaba’s LedgerDB are commercially available verifiable databases that use Merkle trees (or variants) internally to provide transparency logs. VeritasDB uses trusted hardware (SGX) to aid verification. The key difference between such databases and systems like QMDB is that the latter are optimized for frequent state updates and real-time verification of the current state (as opposed to verification of historical logs and deferred verification).

